Self-consistent predictions for LIER-like emission lines from post-AGB stars

Early type galaxies (ETGs) frequently show emission from warm ionized gas. These Low Ionization Emission Regions (LIERs) were originally attributed to a central, low-luminosity active galactic nuclei. However, the recent discovery of spatially-extended LIER emission suggests ionization by both a central source and an extended component that follows a stellar-like radial distribution. For passively-evolving galaxies with old stellar populations, hot post-Asymptotic Giant Branch (AGB) stars are the only viable extended source of ionizing photons. In this work, we present the first prediction of LIER-like emission from post-AGB stars that is based on fully self-consistent stellar evolution and photoionization models. We show that models where post-AGB stars are the dominant source of ionizing photons reproduce the nebular emission signatures observed in ETGs, including LIER-like emission line ratios in standard optical diagnostic diagrams and H$\alpha$ equivalent widths of order 0.1-3 angstroms. We test the sensitivity of LIER-like emission to the details of post-AGB models, including the mass loss efficiency and convective mixing efficiency, and show that line strengths are relatively insensitive to post-AGB timescale variations. Finally, we examine the UV-optical colors of the models and the stellar populations responsible for the UV-excess observed in some ETGs. We find that allowing as little as 3% of the HB population to be uniformly distributed to very hot temperatures (30,000 K) produces realistic UV colors for old, quiescent ETGs.

==> notes.tex <==


% ------ post-AGB / HPHB ---------------
\citet{Rosenfield+2012}

\citet{Brown+2008} - M32 number counts. UVX from EHB stars, not pAGB stars (Small fraction of HB population is hot enough to produce significant UV emission, but most of the UV emission comes from EHB and AGB-manquee stars, implying that post-AGB stars are not a significant source of UV emission even in elliptical galaxies with a weak UV excess).
\citet{Smith+2012} FUV-NUV: Interpreting this colour is complicated, however, since it mixes the effects of the main-sequence turn-off, in the near-UV, with the variation in the hot post-red giant branch content dominating the FUV.
\citet{Weston+2010} - galactic halo
\citet{Girardi+2007} - LMC/SMC
\citet{Pastorello+2013}: SAURON obs of M31 and M32 bulge to ID PNe.
"Considering that the nuclear stellar population of M31 is characterized by a larger stellar metallicity and a much stronger far-UV excess compared to what is found in the central (within one effective radius) regions of M32, the previous results would appear to support the idea that a larger metallicity (which enhances the stellar mass loss efficiency in the RGB) can lead to an HB population that is more tilted towards less massive and hotter He-burning stars, so that its progeny consists mostly of UV-bright AGB-manque stars, but few, if any, bright PNe. A lack of bright PNe is also consistent with the recent reports by Rosenfield et al. (2012) on a shortage of post-AGB stars towards the nucleus of M31, since bright PNe are powered by central postAGB stars. "

% ---
My models indicate you need high Z to get UVX or a population of EHB stars. If EHB stars are more likely at high metallicity, and if this also corresponds to a decrease in post-AGB stars, then we might expect an anti-correlation between strong LIERs and UV upturn galaxies.
That said, the models also indicate that PAGB phase not that sensitive to mass loss efficiency? Changes timescales but time-integrated properties don't change much?
% --------------------------------------
\citet{Trager+2008}: stellar population parameters of elliptical galaxies in the Coma Cluster. SSPs with ages 5-8 Gyr (contrary to predictions from cosmic downsizing).

\citet{Graves+2007}: Compared ETGs with and without LIER-like emission lines. LIER ETGs have younger ages by 2-3 Gyr for the same velocity dispersion.

\citet{Yan+2006}: 30\% of SDSS ETGs have emission lines characteristic of LINERs. Bimodal distribution of OII/Ha EW.

\citet{Yi+2005,Kaviraj+2007,Schawinski+2007}: NUV photometry of SDSS ETGs; morphologically selected galaxies have similar optical colors but a wide range of NUV-optical colors.


% --------- UV upturn -----------------------
Bertola 1982, Brown 1997
\citet{Hernandez+2014}: FUV-NUV, NUV-r colors for UV-upturn galaxies, need binary models.

% --------- Blue HB stars -------------------
Lee, Yoon & Lee 2000
Schiavon et al. 2004
Percival & Salaris 2011
Moehler 2002,2004, 2007 - omega cen extreme HB (T 30,000-50,000K)
Catelan 2009 - HB review
Yaron 2018

% --------- ETG comparisons -----------------
\citet{Renzini+2006}: ETG review on stellar populations. Color (U-V) vs. Magnitude (M_V) relation for elliptical galaxies is very tight. Old ages (over 10 Gyr) and alpha-enhancement required to explain extreme Mg2 line index strength.
\citet{Thomas+2005}: average SFHs for ETGs.
\citet{Choi+2014} Full spectrum fitting of ETGs.

\citet{Burstein+1988}: UV to optical color (UV upturn strength) and Mg2 line strength
\citet{Bureau+2011}: NUV, FUV, optical, Mg, Hb SAURON galaxies

\citet{Smith+2012}: optical and UV colors of ellipticals in Coma Cluster. FUV-NUV < 0.9 is classical UV upturn. Disagree with the \citet{Burstein+1988} and \citet{Bureau+2011} results that FUV-optical color correlates with metallicity. Instead it is an age dependence, and the metallicity is the weaker residual trend. UV upturn in 10\% of ETGs. FUV upturn is caused by helium-burning stars with very thin hydrogen envelopes, with high effective temperatures (EHB, thought also called hot sub-dwarfs since there can be a wide range in formation mechanisms). post-HB evolution can include long-lived UV luminous phases like failed AGB phase, agb-manquee). Yi+2007b. are single star models where enhanced efficiency of mass loss on the red giant branch leads to low envelope mass and high T on the HB. post-HB: more high-metallicity stars follow AGB manquee path instead of AGB branch. Metallicity primarily affects the age at which the rapid UV boost occurs. Han + 2007: EHB form through binary interactions, and FUV vs optical colours are weakly dependent on age for an SSP. Inderect correlations: hot stars responsible for the FUV excess are too faint at optical wavelengths to contribute substantially to the spectroscopic indices. but NUV -- same stars warm main sequence turn-off stars are expected to contribute to the NUV color variations and the spectroscopic ages. ** most of the observed scatter in the NUV vs optical color is a combination of variation in age and metallicity, and a significant contribution from the same hot old stars which dominate the FUV scatter,  and minor contributions from abundance ratio effects and variation in SFH. no need to invoke widespread residual SF to explain the NUV color scatter.

\citet{Schombert} The NUV colors have unusual behavior near u with an inverse CMR and up-and-down signature in two-color diagrams. This indicates a decrease in the UV upturn to intermediate luminosity ellipticals, then a strengthening to higher masses. Models with BHB tracks can reproduce this behavior and match the globular cluster colors, indicating UV upturn is a metallicity effect.

Simplistically, the FUV − NUV colour should be sensitive instead to the temperature of the upturn sources, which would provide further constraints on the origin of the upturn. For instance, Figure 14 of Yi et al. (1997b) shows that within their model, the post-EHB stars generate more FUV flux than the EHB itself, while in the NUV the contributions of EHB and post-EHB are comparable.
In practice however, any attempt to extract information from the FUV − NUV colour alone will be confused by its sensitivity to at least three influences: (i) the age and metallicity of the pre-HB stellar population, via the main-sequence turn-off, (ii) the overall strength of the UV-upturn population, and (iii) the spectral slope of the upturn. In particular the strong observed FUV − NUV correlations likely arise from a compounding of effects (i) and (ii): increasing age and metallicity have the effect of suppressing the NUV flux from the main sequenc

% ----- LINER IONIZATION SOURCES -----------
Central AGN: \citet{Ferland+1983, Halpern+1983, Ho+1999, Kewley+2006, Ho+2009}
Shocks: \citet{Koski+1976, Dopita+1995, Allen+2008}
Accretion of warm gas in cooling flows: \citet{Heckman+1981}
Post-AGB stars as ionization source: \citet{Binette+1994, Taniguchi+2000}

% ----- LINER HISTORY ----------------------
LINER Review: \citet{Filippenko+2003}
Extended multiple kiloparsecs (long slit): \citet{Goudfrooij+1994, Maccehetto+1996}
LINER coined: \citet{Heckman+1980}

% ------ STELLAR STUFF -----------
Lee+1994: metal-poor HB stars can be hot and make good UV sources when they are old
Greggui & Renzini (1990): extremely low-mass HB stars may completely skip AGB; AGB manquee.
Ferguson&Davidsen 1993: PAGB stars should account for 10-30\%

%------------

The nebular model used here is fully integrated within \FSPS and can be easily accessed via the python interface, \pFSPS\footnote{available at \url{http://dan.iel.fm/python-fsps/}}. Users who want to include nebular line and continuum emission in their computed SED can simply set {\tt add\_neb\_emission=True} when initializing the {\tt StellarPopulation} object, modifying the ionization parameter and gas phase metallicity with {\tt gas\_logu} and {\tt gas\_logz}. Complete usage instructions can be found at \url{http://nell-byler.github.io/cloudyfsps/}, including examples for generating mock galaxy spectra with nebular emission as a function of ionization parameter.

Emission line diagnostics like the Baldwin-Philips-Terlevich diagram \citep[BPT; ][]{BPT} are a common way of studying ionized gas and distinguishing the type of ionizing radiation. In these diagrams, star forming galaxies fall in a defined sequence that is well-separated from AGN. In the BPT diagram, the region between the star-forming sequence and the AGN sequence is occupied by objects with emission characterized by strong low-ionization forbidden lines (e.g., \nii{}, \sii{}, \oii{}, \oi{}) relative to recombination lines.


NOTES FROM JIEUN'S PAPER:
The post-AGB timescales in the MIST models (adopting the definition from Miller Bertolami 2016) are consistent with those reported by Miller Bertolami (2016) and Weiss & Ferguson (2009), which are a factor of 3–10 shorter compared to the older post-AGB stellar evolution models (Vassiliadis & Wood 1994; Blöcker 1995). High mass stars are not included because they do not go through the same set of evolutionary phases featured here. The TPAGB and post-AGB phases are not shown for a subset of the models that do not completely evolve through those evolutionary stages. Unsurprisingly, the lifetimes generally decrease with increasing mass, though there are some notable exceptions including the peak in CHeB and AGB lifetimes at ∼ 2 M(see the discussion below).


Johanssen 2016
* SII/Ha > 0.2 means diffuse gas
* electron density of something like 100-150 cm-3
*

In particular, Woods & Gilfanov (2013) demonstrated
that accreting, nuclear-burning white dwarfs would, in the
canonical “single-degenerate scenario” for the production of
type Ia supernovae (SNe Ia), necessarily provide the dominant
contribution to the ionizing background supplied by
old stars. U

In particular, accreting, steadily nuclearburning
white dwarfs (WDs) are expected to number in the
hundreds to thousands within a typical elliptical galaxy (e.g.
Chen et al. 2014). With photospheric temperatures on the
order of ≈1.5–10×105K and spectra well-approximated by
blackbodies (in particular, without any sharp cutoff at the
H I or He II ionization edges, see Rauch & Werner 2010;
Woods & Gilfanov 2013), accreting WDs could in principle
constitute an important part of the ionizing background in
early-type galaxies.

\citet{Johansson+2016} -- coadded SDSS spectra of galaxies with no star formation and AGN. Ha eq of 1.3 ang. Looked for HeII4686 line (progenitors of SN ia).
WHAN-diagram from Cid Fernandes 2011 -- selects on NII and EW(Ha) -- log EW (-0.5-0.5).

\citet{Gomes+2016, Belfiore+2016} -- Stellar population models predict Halpha equivalent widths of 0.5-3 ang.

\citet{Pandya+2017} MASSIVE survey -- warm ionized gas with emission line ratios and equivalent widths consistent with gas excited by old stellar populations. Gas excitation is likely photoionization from evolved stars and fast shocks on extended kpc scales with possible additional contributions from low-luminosity AGN on nuclear scales. 

\citet{Hirschmann+2017} - a version of self-consistent modelling.

\citet{Singh+2013}The most probable explanation for the excess LINER-like emission is ionisation by evolved stars during the short but very hot and energetic phase known as post-AGB. This leads us to an entirely new interpretation. Post-AGB stars are ubiquitous and their ionising effect should be potentially observable in every galaxy with the gas present and with stars older than ~1 Gyr unless a stronger radiation field from young hot stars or an AGN outshines them. This means that galaxies with LINER-like emission are not a class defined by a property but rather by the absence of a property. It also explains why LINER emission is observed mostly in massive galaxies with old stars and little star formation.

\citet{Gomes+2016} - CALIFA galaxies, EW estimates for LIER like emission. Estimate theoretical EWs from stellar population models Method takes the SSPs associated with the best-fit model, and integrates the SEDs blueward of the lyman continuum limit. SSPs with ages > 10^8 predict the Ly-c output of the pAGB component only; balmer line luminosities are then computed assuming case B recombination and standard conditions for the gas (n=100; T=10^4k).

 Since it is now recognized that LINER-specific emission-line ratios
are not confined to galaxy nuclei (e.g., Sharp & Bland-Hawthorn,
2010; Kehrig et al., 2012; Papaderos et al., 2013; Singh et al., 2013), a
more adequate acronym would be low-ionization emission-line regions
(LIERs).

Likewise, Eracleous et al. (2010) point
out that pAGB stars provide more ionizing photons than AGN
in more than half of the LINERs and can account for the observed
line emission in 1/3 of these systems. 

As
Stasinska et al. ´ (2008) argue, a significant fraction of ETGs are
in fact ‘retired’ galaxies, i.e. systems that stopped forming stars,
and whose ionizing field is powered solely by pAGB sources.

the presence or
absence of LINER characteristics as an argument for or against
pAGB photoionization, since it is known that they can be due to
a variety of mechanisms, including shocks and starburst-driven
outflows (see, e.g., Sharp & Bland-Hawthorn, 2010, for a recent
observational review).


For early-type galaxies where the bulk of the stellar population is old, post-AGB stars can contribute a significant portion of the total galaxy luminosity. Post-AGB stars are not capable of matching the ionizing flux produced by a single O-star; their strength lies in numbers. The progenitors of these stars have initial masses from 1-5\Msun{}, and are much more common than O-type stars.

%In Fig.~\ref{fig:ionSpec} we show example ionizing spectra for instantaneous bursts at different metallicities. The top panel shows ionizing spectra for 100\Myr instantaneous bursts ($\log t = 8$) to highlight the contribution from the hot horizontal branch stars, which can be seen as an increase in flux in between the ionization energy for helium, I$_{\mathrm{He}}$, and the ionization energy for hydrogen, I$_{\mathrm{H}}$. These stars are hotter in lower metallicity populations, with their strongest contribution seen in the stellar population with \logZeq{-2}.

%The onset of the first post-AGB stars varies with metallicity. The bottom panel of Fig.~\ref{fig:ionSpec} shows ionizing spectra for 2\Gyr instantaneous bursts; at 2\Gyr post-AGB stars are present at all metallicities. The spectra blueward of I$_{\mathrm{H}}$ appear clustered due to the fact that there are only two metallicities in the spectral library used for post-AGB stars.


The region of the BPT diagram between the star-forming sequence and the AGN sequence is occupied by objects classified as ``low ionization emission regions''\citep[LIERs, ][]{Belfiore16}\footnote{Low ionization nuclear emission regions \citep[LINERs, ][]{Heckman1980} refers to centrally concentrated low ionization emission, which are likely attributed to weak AGN-related activity.}. LIER-like emission is characterized by strong low-ionization forbidden lines (e.g., \nii{}, \sii{}, \oii{}, \oi{}) relative to recombination lines, and was originally discovered in the nuclear regions of galaxies and attributed to AGN-related activity \citep{Kauffmann03b, Kewley06, Ho08}. While some cases are certainly still driven by the presence of a weak AGN, the discovery of spatially extended (${\sim}$kpc scales) LIER-like emission has led to work suggesting that hot, evolved stars could be responsible for the ionizing radiation in other cases \citep{Singh13, Belfiore16}. The leading candidate for the ionizing source is the population of post-AGB stars \citep{Binette94, Sarzi10, Yan12}. Extreme horizontal branch stars have also been suggested candidates, but considering their effect is beyond the scope of this paper.

Post-AGB stars are stars that have left the AGB, evolving horizontally across the HR diagram towards very hot temperatures ($\sim10^5$ K) before cooling down to form white dwarfs, with a fraction of the post-AGB population forming planetary nebulae. The exposed cores of post-AGB stars are hot enough to ionize hydrogen and thus could produce a radiation field capable of ionizing the surrounding ISM, provided that there are enough post-AGB stars. 

Post-AGB stars are not capable of matching the ionizing flux produced by a single O-star; their strength lies in numbers. The progenitors of these stars have initial masses from 1-5\Msun{}, and are much more common than O-type stars. For early-type galaxies where the bulk of the stellar population is old, AGB and post-AGB stars can contribute a significant portion of the total galaxy luminosity. \citet{Yan12} measured the ionization parameter and gas density for galaxies with LIER-like emission and compared it to the typical numbers of ionizing photons produced by post-AGB stars. They deduced that the ionization parameter for post-AGB stars falls short of the required value by a factor of 10, implying that the gas geometry must be quite close to the stars themselves.

%-------------------------------------------------------
% pAGB BPT Rinner, nH
%-------------------------------------------------------
\begin{figure}[!htbp]
  \begin{centering}
    \includegraphics[width=0.45\textwidth]{f27.pdf}
    \caption{BPT diagram for an ionizing spectrum produced by a 3 Gyr solar metallicity SSP that includes post-AGB stars. The grayscale 2D histogram is star forming galaxies from SDSS. The solid black line shows the extreme starburst classification line from \citet{Kewley01} and the dashed line is the pure star formation classification line from \citet{Kauffmann03a}. Our old-star models with post-AGB stars do produce line ratios consistent with LIER-like emission, but large numbers of post-AGB stars (at least M$_{\mathrm{initial}} \sim 10^6\Msun{}$) would be required to produce enough ionizing photons.}
    \label{fig:pAGBBPT}
  \end{centering}
\end{figure}
%-------------------------------------------------------

The geometry between the stars and gas is one of the major uncertainties associated with interpreting LIER-like emission. We first determine if populations including post-AGB stars are capable of producing line ratios consistent with LIER-like emission. The geometry previously assumed in this work ($\logR = 19$; $\nH = 100$) is appropriate for massive \hii regions found in star forming galaxies, where the gas is associated with the natal gas cloud, butmay not accurately describe the gas geometry in a scenario where old stars provide the ionizing radiation.

To test the sensitivity to geometry, we generate ionizing spectra for older SSPs ($>1$ Gyr) that include post-AGB stars to use as input to \Cloudy, and run photoionization models at different values of \Rin{} and \nH{}. In \Fig{pAGBBPT} we show the BPT diagram line ratios for the post-AGB star ionizing spectra at several different ionization parameters, with \nH varied from 10-1000 and the inner radius varied from $10^{18}-10^{20}$ cm (0.3-30 pc). 

The post-AGB models produce line ratios consistent with LIER-like emission, well outside of the ``pure star forming'' region of the BPT diagram, as identified by \citet{Kauffmann03a}. The ionization parameters required to produce observable line ratios are $\logU \sim -5$ to  $\logU \sim -3$. At $\Rin=10^{19}$ and $\nH=100$ cm$^{-3}$, this implies a total initial stellar mass of $10^6$-$10^8\Msun$. The required stellar mass would be higher for models where the inner radius is further from the ionizing source. We note that the ionizing spectrum was based on a stellar population at solar metallicity; low-metallicity post-AGB stars are hotter and would likely enhance the ionizing radiation.

The line ratios in \Fig{pAGBBPT} show little sensitivity to the star-gas geometry, a result of our simplified model in which the gas exists in a plane-parallel shell surrounding a central point source of ionizing radiation. If the gas is produced by the AGB stars themselves or has a spatial distribution that differs from the distribution of stars, the geometry will differ substantially from the simplified shell used in this work. In future work we plan to test the effects of model geometry in more detail. 

%-------------------------------------------------------
% pAGB spectrum
%-------------------------------------------------------
\begin{figure}[!htbp]
  \begin{centering}
    %\plotone{f26a.pdf}
    %\plotone{f26b.pdf}
    \includegraphics[width=0.45\textwidth]{f28a.pdf}\\
    \includegraphics[width=0.45\textwidth]{f28b.pdf}
    \caption{\textbf{Top:} The effect of hot, evolved stars on the ionizing spectrum. The default default spectrum for a 3 Gyr SSP at solar metallicity is shown shown in black. The weight of the post-AGB phase is modulated from 1 (full inclusion of post-AGB stars) to $10^{-4}$, which decreases the amount of EUV flux relative to the rest of the population. \textbf{Bottom:} BPT diagram for photoionization models where \U{} and the weight of the post-AGB phase are varied. The solid black line shows the extreme starburst classification line from \citet{Kewley01} and the dashed line is the pure star formation classification line from \citet{Kauffmann03a}. The grayscale 2D histogram shows the number density of SDSS star-forming galaxies. The \citet{Vassiliadis} tracks used for post-AGB stars must be correct within a factor of two if post-AGB stars are responsible for LIER-like emission.}
    \label{fig:hotstars}
  \end{centering}
\end{figure}
%-------------------------------------------------------

Another major uncertainty associated with the interpretation of LIER-like emission lies in our incomplete understanding of the late stages of stellar evolution. In addition to the poor constraints on the age distribution and lifetimes of post-AGB stars, it is uncertain what fraction of post-AGB stars contribute to the large-scale photoionizing radiation field. A recent census of the old, UV-bright stellar population in M31 was unable to reproduce predicted numbers of post-AGB stars \citep{Brown2008}. 

To understand the sensitivity of LIER-like emission to the underlying stellar model, we generate ionizing spectra with varying contribution from post-AGB stars using the {\tt pagb} parameter in \FSPS. This parameter specifies the weight given to the post-AGB star phase, where {\tt pagb=0.0} turns off post-AGB stars and {\tt pagb=1.0} implies that the \citet{Vassiliadis} tracks are implemented as-is, the default behavior in \FSPS. In the top panel of \Fig{hotstars} we show the ionizing spectrum produced by a 3 Gyr SSP with {\tt pagb} set to 1, $10^{-1}$, $10^{-2}$, and $10^{-3}$. Scaling down the implemented post-AGB stars scales down the emergent EUV radiation in the spectrum.

We show the resultant BPT diagram for the photoionization models that vary in both \U{} and {\tt pagb} in the bottom panel of \Fig{hotstars}. We find that the luminosity of the post-AGB stars could be reduced by a factor of two and still produce LIER-like emission, provided there are enough stars.

\citet{Belfiore16} found that the \sii{}/\ha{} line ratio provided a clean separation between LIER-like emission and Seyfert-like emission. In \Fig{lier}, we show the \sii{} emission produced by our post-AGB models. The line ratios produced by our post-AGB star models show the elevated \sii{}/\ha{} ratios observed in LIER galaxies, and confirms the utility of \sii{} as a means of identifying low-ionization emission.

%-------------------------------------------------------
% pAGB spectrum
%-------------------------------------------------------
\begin{figure}[!htbp]
  \begin{centering}
    %\plotone{f27.pdf}
    \includegraphics[width=0.45\textwidth]{f29.pdf}
    \caption{\sii{}/\ha{} versus \oiiihb{} diagnostic diagram. Ionization parameter varies from $\U=-1$ (dark blue) to $\U=-4$ (light blue), and the weight of the post-AGB stars is varied (purple to yellow). The grayscale 2D histogram shows the density of star-forming galaxies and the black line shows the pure star formation classification line from \citet{Kauffmann03a}. The old star models that include post-AGB stars are able to reproduce the elevated \sii{}/\ha{} emission observed in LIERs.}
    \label{fig:lier}
  \end{centering}
\end{figure}
%-------------------------------------------------------

%-------------------------------------------------------
% EvType QH vs time for logZ=-2
%-------------------------------------------------------
\begin{figure}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{EvType_m200_QH.png}\\
    \includegraphics[width=0.48\textwidth]{EvType_m200_QHe.png}
    \caption{\emph{Top}: The ionizing photon flux per unit stellar mass, \QHat, as a function of time for different stellar types at 1\% solar metallicity. \emph{Bottom}:The ionizing photon flux per unit stellar mass for Helium, \QHe as a function of time for different evolutionary phases. In very metal poor populations, hot horizontal branch stars provide additional ionizing radiation. These stars provide significant amounts of hydrogen ionizing photons but are not hot enough to produce significant numbers of helium-ionizing photons.}
    \label{fig:m2QF}
  \end{center}
\end{figure}
%-------------------------------------------------------
%For very metal-poor populations (\logZeq{-1.5} and below) hot horizontal branch stars can also contribute to the ionizing photon flux. Stars that begin their horizontal branch evolution with larger hydrogen envelopes have hydrogen-shell burning in addition to core-He burning, making these stars hotter and bluer. Metal-poor stars lose less mass on the RGB, retaining larger hydrogen envelopes, producing hotter HB stars. In Fig.~\ref{fig:m2QF} we show the same plots from Fig.~\ref{fig:QF}, but for a stellar population with \logZeq{-2}. The horizontal branch stars (Core He-Burning or \emph{CHeB}) contribute hydrogen-ionizing photons between 10-100\Myr. These hot horizontal branch stars contribute significant amounts of hydrogen-ionizing photons but are not hot enough to produce many helium-ionizing photons.

==> other_figs.tex <==
%These different subclasses include stars with a range of temperatures, luminosities, and lifetimes, not all of which are equally effective at driving ionization. They can however, produce significant UV flux longwards of 912\ang, even for old stellar populations. This flux has been detected with facilities like GALEX, SWIFT, or IUE at low redshift, or with optical or NIR facilities for highly redshifted galaxies. In some cases the UV flux is seen to rise towards short wavelengths, in a phenomenon referred to as the ``UV upturn''.
%
%The source of the UV-upturn phenomenon in ETGs is still debated, with suggestions that include a population of helium-rich stars or stars who have had their atmospheres stripped away through binary interactions. The manifestation of the UV upturn phenomenon is highly variable, occuring in roughly 3-10\% of local ETGs (depending on selection criteria, see for example \citealp{Smith+2014}), independent of whether the ETG hosts LIER-like emission. Likewise, recent work has found that ETGs with similar morphologies and optical colors can display a wide range of NUV-optical colors \citep{Yi+2005, Kaviraj+2007, Schawinski+2007}. 
%
%All of these UV-emission phenomena in old stellar populations (photoionization to produce LIER-like emission, UV upturn, diverse UV-optical colors) are likely to be driven by stars of similar masses (${\sim}$3, 2, and 1 \Msun for 2, 6, and 12\Gyr old populations) given the rapidity of post-RGB evolution. As such, a self-consistent model of the stellar and nebular spectral energy distribution (SED) should be able to simultaneously reproduce the UV and optical colors and emission line ratios of LIER-like galaxies, if HPHB models are correct.
%
%Calculating the needed self-consistent models of UV emission requires making predictions for the nebular emission produced by ionization from the hottest HPHB phases.
%
%However, these current estimates are first-order calculations assuming case-B recombination for fixed-temperature gas. In \citet{Byler+2017}, we showed that accounting for temperature variations is essential when predicting emission line strengths. Accurate predictions of emission line luminosities and equivalent widths require the consideration of metallicity- and age-driven changes to the ionizing spectrum and metallicity-driven changes in the gas phase abundances. 




\section{Discussion}\label{sec:discussion}


\subsection{UV-optical colors}\label{sec:UV}

The optical properties of ETGs are fairly well characterized. The UV is much more uncertain, however, as galaxies with similar optical colors can have very different UV colors. In this section, we ask if the models from \S\ref{sec:stars} are also able to correctly predict the UV properties of ETGs, while also considering the contribution from other non-ionizing, UV-bright stellar types. Although the evolutionary pathways and lifetimes of these hot, evolved, populations are not well-understood and models of their SEDs are uncertain, comparisons are still informative.

We first consider the UV properties of horizontal branch stars. These stars are not as luminous as post-AGB stars, but are longer-lived and thus more numerous. Blue horizontal branch (BHB) stars typically have temperatures between 7,000 and 20,000K \citep[e.g.,][]{Schiavon+2004}, with the hottest HB stars often referred to as Extreme Horizontal Branch (EHB) stars (\Teff$>20,000$\,K). Even a modest population of BHB stars can significantly alter the UV colors of a stellar population. However, temperatures in excess of 15,000K are required to ionize hydrogen, and thus only in the most extreme cases will HB stars contribute significantly to the ionizing photon budget.

BHB stars are not included by default in \FSPS, but they can be added in using the {\tt fbhb} parameter, which specifies the fraction of horizontal branch stars that are blue. In the standard implementation, \FSPS redistributes the specified fraction of HB stars such that they are uniformly spread in $\log T_{\mathrm{eff}}$ up to $10^4$\,K \citep[e.g.,][]{Sarajedini+2007}. However, HB star temperatures have been observed in excess of $10^4$K (e.g., \citealt{Dalessandro+2013}, also \citealt{Catelan+2009}). To include the most extreme cases we increase the {\tt fbhb} temperature limit to $10^{4.5}$ K (${\sim}$30,000$\,$K, the limit of a B-type star). There are a few observations of EHB stars with temperatures in excess of 30,000\,K \citep[][and references therein]{Moehler+2007}, however, the hottest of these stars likely represent extreme evolutionary pathways \citep[e.g., extreme He-enhancement or pop II stars, see][]{Yaron+2017} and will not be representative of the typical old stellar populations observed in ETGs locally.

We generate SEDs for models where we vary {\tt fbhb} from 0 to 1. A model with {\tt fbhb}$=1$ implies that 100\% of the stars flagged as horizontal branch stars have had their temperatures uniformly redistributed up to $\Teff=10^{4.5}$K.

To demonstrate the different UV properties of post-AGB and BHB stars, we show the SEDs from different 3\Gyr SSPs between 300 and 3000\ang in the left panel of Fig.~\ref{fig:UV}. The fiducial solar metallicity model is shown with a solid yellow line, while the 10\% solar metallicity model is shown with a dashed blue line. Models run with {\tt fbhb}$=0.1,0.5,1$ are shown in progressively darker purples. The presence of even a small number of BHB stars can dramatically change the UV colors of a population. The BHB stars produce significantly more FUV flux than the fiducial model at both solar and sub-solar metallicities. The inclusion of these hot horizontal branch stars has no discernible affect on the predicted ionizing photon budget, though we note that this may not be true for other, generative HB models \citep[e.g.,][]{Yaron+2017}.

% want to say something about FUV/NUV is nearly constant -- optical -UV color will largely ineff. would swift filter give better leverage?

%-------------------------------------------------------
% UV colors
%-------------------------------------------------------
\begin{figure*}
  \begin{center}
    \includegraphics[width=\textwidth]{figs/f8.png}
    \caption{{\sc UV properties of hot, evolved stars} -- \emph{Left:} The total SED from $800-3000$\ang. The fiducial post-AGB star model at solar metallicity is shown in yellow and 10\% solar metallicity is in blue, for a $\tau=0.5$\Gyr model at 10\Gyr. The purple lines show models where the fraction of BHB stars is modified from the fiducial model. The presence of BHB stars can dramatically change the UV colors of a stellar population, but do not contribute significantly to the ionizing photon flux. \emph{Right:} UV-optical color-color diagram reproduced from \citet{Hernandez+2014}. Each model is plotted as a line, showing how it would appear at different ages as it evolves from 3\Gyr (circle) to 14\Gyr, with colored lines corresponding to the metallicities and BHB fractions from the left panel. The vertical dashed line at $NUV-r=5.4$ separates red-sequence galaxies, and the horizontal line at $FUV-NUV=0.9$ shows the boundary of classic UV-upturn galaxies from \citet{Smith+2014}. The post-AGB stars responsible for nebular emission cannot be wholly responsible for the UV excess in some ETGs. However, even a small population of extreme-HB stars can produce a UV excess-like signature. High BHB fractions produce blue $NUV-r$ colors inconsistent with the general ETG population.}
    \label{fig:UV}
  \end{center}
\end{figure*}
%-------------------------------------------------------

The right panel of Fig.~\ref{fig:UV} is a reproduction of Fig.~1 from \citet{Hernandez+2014}, which shows the $FUV-NUV$ \emph{\vs} $NUV-r$ colors of the $\tau=0.5$\Gyr ETG models from \S\ref{sec:stars:continuum} between 3 and 14\Gyr, highlighting the youngest age with a circular marker. The galaxy colors include the contribution from nebular line and continuum emission, assuming an ionization parameter of \logUeq{-4}. The color scheme is identical to the left panel of Fig.~\ref{fig:UV}, where yellow and blue lines represent models at solar and 10\% solar metallicity, respectively. The progressively darker purple lines show models where {\tt fbhb} has been increased from 0 to 0.1, 0.5, and 1.0.

The grey points in Fig.~\ref{fig:UV} are the ETG sample from \citet{Hernandez+2014}. The vertical dashed line at $NUV-r=5.4$ is their galaxy red sequence limit and the horizontal line at $FUV-NUV$ = 0.9 shows the limit for selection of classical UV-upturn galaxies. Galaxies on the red sequence that fall below this line are said to have a ``UV excess'' (UVX) \citep{Smith+2014}. Galaxies below this line but on the blue side of the red sequence division are thought to have blue colors originating from residual star-formation (RSF), rather than canonical UVX emission. Our models with $\tau > 0.5$ (not plotted) fall into this region.

\citet{Hernandez+2014} found it difficult to generate models in the UVX portion of the UV color-color diagram without invoking binary star interactions, which can strip the outer envelope of a star, making it appear hotter. Without the BHB, our models are able to populate the UVX portion of Fig.~\ref{fig:UV}, but only at high metallicity, and none of our models reach the most extreme portion of the UVX region.

Including a BHB improves the situation by moving the models towards bluer $FUV - NUV$ colors, towards the center of the observed ETG locus. Even a small fraction of BHB stars (${\sim}10$\%) can successfully move the model into the UVX portion of the diagram. However, once BHB stars are present, $FUV-NUV$ does not change significantly, and increasing {\tt fbhb} largely moves the models to bluer $NUV-r$ colors at similar $FUV-NUV$ colors. Thus, the BHB stars considered here do not produce the necessary FUV flux to fully explain the observed range of UVX colors, suggesting a need for hotter BHB populations. Furthermore, as {\tt fbhb} increases, the bluer $NUV - r$ colors become incompatible with the bulk of the ETG population.

We note that the BHB implementation in \FSPS redistributes stars uniformly across the horizontal branch in temperature, and models with only BHB or EHB stars could produce the necessary FUV flux needed to move the baseline models into the UVX region.

%The fiducial solar-metallicity model is not blue enough in the $FUV-NUV$ color. The solution requires flux added primarily to the FUV filter with little flux added to $NUV$ and $r$ filters. Post-AGB stars don't contribute enough flux and are too hot to adequately reproduce the UV excess. Stars with temperatures between 20,000 and 30,000K, typical for EHB stars. The current implement
%You could maybe just plot a single black body on the left hand panel to show the type of temperature that would add flux to FUV but not much to NUV or r. You could then even invert the discussion by first comparing the no BHB models to the data and argue “here’s the SED and color color diagram of ETGs with no BHBs. Not blue enough. solution requires adding FUV flux primarily. The pAGB stars (plotted) don’t contribute enough flux and are too hot.  Stars of 25000k (or whatever) would do the trick and are the max temp of EHB stars. FSPS does have BHb implementation. Doesn’t currently allow fixed temp but does let us explore typical overall flux contribution. Overall flux is in ballpark for even small 10% fraction, but continuous temp distribution is too flat. Suggests modest fix to bimodal temp might work.”


In the current implementation, neither BHB or EHB stars produce enough ionizing radiation to lead to LIER-like emission. This points to a scenario where the post-AGB stars produce the ionizing radiation necessary for LIER-like emission, while a different population of HPHB stars drive the FUV and NUV behavior.

It is interesting to consider the possibility of an anti-correlation between UVX objects and LIER-like emission strength. While the detailed evolutionary paths of HPHB stars remain an ongoing source of debate, some have suggested that extreme HB stars are failed AGB stars that immediately evolve through to the WD cooling sequence, reducing the population of post-AGB stars. This has been invoked to explain the relative paucity of post-AGB stars observed in M31, where high metallicities are thought to produce an enhanced population of extreme HB stars. In this scenario, the enhanced EHB population would produce a strong UV-excess, while the reduced post-AGB population would reduce LIER-like emission and thus \ha equivalent widths.










\subsection{Optical colors} \label{sec:stars:continuum:colors}

In Fig.~\ref{fig:optCols} we show the SDSS $u-r$ \vs $r-z$ color-color diagram for our models at a range of ages and metallicities, for stellar-only models (\emph{bottom row}) and stellar+nebular emission models (\emph{top row}, assuming \logUeq{-4}). The $u-r$ \vs $r-z$ diagram has proven to be an efficient means of selecting quiescent, red-sequence ETGs. The \citet{Holden+2012} boundary for selecting quiescent ETGs is indicated with the black dotted line; the \citet{McIntosh+2014} extension for ``recently quenched'' ETGs is shown with the black solid line. In general, the inclusion of nebular emission has little affect on the optical colors. For instantaneous bursts (\emph{left column}), models with metallicities richer than \logZeq{-1} and ages older than $\sim2$\Gyr have optical colors that are appropriate for the ETG population.

Columns two and three of Fig.~\ref{fig:optCols} show the same color-color diagrams for the delayed-$\tau$ models, for $\tau = 0.5$ and 1.0\Gyr, respectively. The models with $\tau=0.1$\Gyr are essentially indistinguishable from the instantaneous bursts, and are thus ommitted from Fig.~\ref{fig:optCols}. The $\tau=0.5$\Gyr models show qualitatively similar behavior to the instantaneous bursts. The $\tau=1$\Gyr models are much bluer than the instantaneous bursts, and only the most metal rich models produce colors consistent with the red, quiescent galaxy population.

%-------------------------------------------------------
% Optical Colors
%-------------------------------------------------------
\begin{figure*}
  \begin{center}
    \includegraphics[width=\linewidth]{figs/f9.png}
    \caption{Optical color-color diagram for stellar populations using a delayed$-\tau$ model SFH, with $\tau=0.0$\Gyr (instantaneous burst, \emph{left}), $\tau=0.1$\Gyr (\emph{middle}), and $\tau=0.5$\Gyr (\emph{right}). The top row shows models that include nebular emission, with \logUeq{-4} while the bottom row shows models that do not include nebular emission. Models with ages between 1 and 13\Gyr are plotted, color-coded by metallicity. Age is indicated by the transparency of the points, with the 13\Gyr model points fully opaque. The SDSS $u-r$ \vs r-z colors efficiently separate blue, star-forming galaxies from quiescent, red galaxies. The black line selects ETGs from \citet{Holden+2012}, revised by \citet{McIntosh+2014} to include recently quenched ETGs. The models used in this work have optical colors representative of the general ETG population.}
    \label{fig:optCols}
  \end{center}
\end{figure*}
%-------------------------------------------------------

\subsection{Lick indices} \label{sec:stars:continuum:lick}

The Lick/IDS line strength system \citep{Worthey+1994, Trager+2000} leverages specific spectral features in the optical spectrum that correlate with the age and metallicity of a stellar population. For elliptical galaxies with old stellar populations, stars with initial masses between 1 and 2\Msun dominate both the optical spectrum and the ionizing radiation responsible for LIER-like emission. In this section, we show that our models with nebular emission still produce Lick indices consistent with the general ETG population.

We use Lick definitions from \citet{Vazdekis+2010}. We compare our models to the \hb Lick index and the [MgFe] index, a combination of several Lick indices (\texttt{Mg\_b}, \texttt{Fe5270}, and \texttt{Fe5335}) which is sensitive to metallicity, where higher metallicity populations produce larger values of [MgFe]. The [MgFe] index is also relatively insensitive to $\alpha-$abundance enhancements. To calculate [MgFe], we use the definition from \citet{Galleti+2009}:
\begin{equation}
    [\mathrm{MgFe}] = \sqrt{\texttt{Mg\_b} \times \frac{\texttt{Fe5270} + \texttt{Fe5335}}{2}}.
\end{equation}

In Fig.~\ref{fig:LickMgFe} we show the [MgFe] index compared to the optical SDSS $g-r$ color for our ETG models at different metallicities. As in Fig.~\ref{fig:optCols}, the bottom row shows models without nebular emission, while the top row shows models that include both nebular line and continuum emission, assuming \logUeq{-4}, typical for LIER-like galaxies. Each column shows a different delayed$-\tau$ model, from $\tau=0$\Gyr (instantaneous burst, \emph{left column}) to $\tau=1$\Gyr (\emph{right column}). The grey shaded region indicates the location of elliptical galaxies and ancient, massive, globular clusters (GCs) from \citet{Schombert+2016}.

Our models produce reasonable [MgFe] values, consistent with the low-metallicity GCs and the more metal-rich ETGs. For the $\tau=1$\Gyr model, the extended SF changes the $g-r$ colors significantly until $\sim5$\Gyr, after which the [MgFe] and $g-r$ colors are consistent with the observed ETGs. The [MgFe] indices do not cover spectral regions with any strong nebular emission lines, thus, the models with and without emission are very similar for models at late ages.

In Fig.~\ref{fig:LickHb} we show the age-sensitive \hb Lick index compared to the optical SDSS $g-r$ color in the same style as Fig.~\ref{fig:LickMgFe}. The \hb index is a well-known age-indicator, decreasing as the stellar population ages. The ETGs and GCs from \citet{Schombert+2016} have \hb between 0 and 4\ang, with \hb decreasing as the $g-r$ color gets redder. Our models with and without emission show similar behavior, with high values and blue colors for young models and low \hb combined with redder colors for models over a few Gyr. Models with ages between $2-13$\Gyr are best matched to the ETG and GC data, with lower metallicities for the GCs and higher metallicities for the ETGs. The models with nebular emission show slightly modified \hb values and colors, though overall still consistent with the data. In the models that include emission, \hb emission causes the \hb index to decreases rapidly while the $g-r$ color stays the same.

In what follows, we will largely restrict our analysis of emission lines and UV emission to the subset of models that are also consistent with the observed properties of ETGs in Figures~\ref{fig:optCols} - \ref{fig:LickHb}.

%-------------------------------------------------------
% optical colors
%-------------------------------------------------------
\begin{figure*}
  \begin{center}
    \includegraphics[width=\linewidth]{figs/f10.png}
    \caption{Optical $g-r$ color and the [MgFe] Lick index for our ETG models with stellar and nebular emission (\emph{top row}) and stellar only emission (\emph{bottom row}). Each column shows a different delayed$-\tau$ model SFH: $\tau=0.0$\Gyr (instantaneous burst, \emph{left}), $\tau=0.1$\Gyr (\emph{middle}), and $\tau=0.5$\Gyr (\emph{right}), and $\tau=1$\Gyr (\emph{bottom row}). Models with ages between 1 and 13\Gyr are plotted, color-coded by metallicity. Age is indicated by the transparency of the points, with the 13\Gyr model points fully opaque. The grey shaded region shows the location of observed objects from \citet{Schombert+2016}, which includes globular clusters and elliptical galaxies. For models with extended SF ($\tau=1$\Gyr), the inclusion of nebular emission alters the $g-r$ color at young ages. After $\sim5$\Gyr the models with nebular emission are consistent with the observed population of ETGs.
    }
    \label{fig:LickMgFe}
  \end{center}
\end{figure*}
%-------------------------------------------------------

%-------------------------------------------------------
% optical colors
%-------------------------------------------------------
\begin{figure*}
  \begin{center}
    \includegraphics[width=\linewidth]{figs/f11.png}
    \caption{Optical $g-r$ color and the \hb Lick index for our ETG models with stellar and nebular emission (\emph{top row}) and stellar only emission (\emph{bottom row}). Each column shows a different delayed$-\tau$ model SFH: $\tau=0.0$\Gyr (instantaneous burst, \emph{left}), $\tau=0.1$\Gyr (\emph{middle}), and $\tau=0.5$\Gyr (\emph{right}). Models with ages between 1 and 13\Gyr are plotted, color-coded by metallicity. Age is indicated by the transparency of the points, with the 13\Gyr model points fully opaque. The grey shaded region shows the location of observed objects from \citet{Schombert+2016}, which includes globular clusters and elliptical galaxies. Nebular emission has an significant impact on the \hb index, since the emission fills in the \hb absorption feature, lowering the index.
    }
    \label{fig:LickHb}
  \end{center}
\end{figure*}
%-------------------------------------------------------



%-------------------------------------------------------
% Total time evolution for QH, QHe at all metallicities
%-------------------------------------------------------
\begin{figure}
  \begin{center}
    \includegraphics[width=\linewidth]{figs/f4.png}
    \caption{\emph{Top}: The ionizing photon flux per unit stellar mass, \QH, as a function of time for stellar populations with metallicities varying from \logZeq{-2} to \logZeq{0.5}. \emph{Bottom}: The ionizing photon flux per unit stellar mass for Helium, \QHe, as a function of time. For young stars, the metal-poor populations have higher ionizing photon rates and extended main-sequence lifetimes. The bump in \QH at $\log t = 7.8$ seen in populations with metallicities below \logZeq{-0.5} is due to hot horizontal branch stars, which are not hot enough to produce a similar bump in \QHe. The large increase in \QHe after $\log t = 8$ is due to the first onset of post-AGB stars.}
    \label{fig:popQs}
  \end{center}
\end{figure}
%-------------------------------------------------------

%===============================================================================
\section{UV emission from hot evolved stars}\label{sec:colors}
%===============================================================================

As discussed in \S\ref{sec:stars:continuum}, there are broad classes of star formation histories that produce reasonable SDSS ETG colors. Thus, the emission line ratios and equivalent widths presented in \S\ref{sec:stars} are relatively model independent, as the optical properties of ETGs are fairly well understood. The UV is much more uncertain, however, as galaxies with similar optical colors can have very different UV colors. In this section, we ask if the models from \S\ref{sec:stars} are also able to correctly predict the properties of other UV populations, including post-AGB stars, hot horizontal branch stars, and blue straggler stars. We note that the evolutionary pathways and lifetimes of these populations are not well-understood and models of their SEDs are uncertain.

In this section we explore the contribution from three main stellar types. We first consider post-AGB stars, which we have shown dominate the ionizing photon budget at old ages and are able to reproduce the emission line properties of LIER-like galaxies. We can vary the contribution from post-AGB stars to the total SED using the {\tt pagb} parameter in \FSPS. This parameter specifies the weight given to the post-AGB star phase, where {\tt pagb=0.0} turns off post-AGB stars and {\tt pagb=1.0} implies that the MIST models are implemented as-is, the default behavior in \FSPS. Models with {\tt pagb} between 0 and 1 have the flux from the post-AGB stars scaled down by {\tt pagb}.

Second, we explore the contribution from hot horizontal branch stars. These stars are not as luminous as post-AGB stars, but are longer-lived and thus more numerous. Blue horizontal branch (BHB) stars typically have temperatures between 7,000 and 20,000K \citep{Schiavon+2004}, with the hottest BHB stars often referred to as Extreme Horizontal Branch (EHB) stars. A modest population of BHB stars can alter the UV colors of a stellar population. However, since temperatures in excess of 15,000K are required to ionize hydrogen, only in the most extreme cases will BHB stars contribute significantly to the ionizing photon budget. BHB stars are not included in the default \FSPS parameters, but they can be included using the {\tt fbhb} parameter, which specifies the fraction of horizontal branch stars that are blue. \FSPS redistributes the specified fraction of HB stars such that they are uniformly spread in $\log T_{\mathrm{eff}}$ to $10^4$K \citep[e.g.,][]{Sarajedini+2007}. However, BHB temperatures have been observed in excess of $10^4$K, to include the most extreme cases we increase the BHB temperature limit to $10^{4.5}$K (${\sim}$30,000$\,$K, the limit of a B-type star) in the following tests.

Finally, we also explore the contribution from blue straggler stars. These are rejuvenated main sequence stars that appear blueward of the main sequence turn-off in globular clusters (GCs). We vary the contribution of these stars in \FSPS using the $S_{\mathrm{BS}}$, or {\tt sbss} parameter, which specifies the specific frequency of blue straggler stars relative to the number of horizontal branch stars ($S_{\mathrm{BS}} = N_{\mathrm{BS}} / N_{\mathrm{HB}}$). This number can be varied between 0 and 10, but is observed to be between 0.1 and 5 in GCs, and its value in ETGs is unknown.

In Fig.~\ref{fig:HPHB} we show an example spectrum from a 3 Gyr SSP at solar metallicity, shown in black. We indicate the ionization energies of hydrogen and helium with the black dashed lines, and show the GALEX FUV and NUV bandpasses in grey. We then systematically vary the {\tt pagb}, {\tt fbhb}, {\tt sbss} parameters from the baseline models.

We show the effect of decreasing {\tt pagb} from 1 to $10^{-1}$, $10^{-2}$, and $10^{-3}$ in orange. Scaling down the implemented post-AGB star contribution scales down the emergent EUV radiation in the spectrum. The MIST models do not include evolutionary pathways for early-AGB or AGB-Manque stars, so varying {\tt pagb} could be interpreted as varying the number of stars evolving through the traditional post-AGB phase. If a substantial fraction of post-AGB stars have untraditional evolutionary pathways, the ionizing photon budget would change significantly.

We show the effect of adding BHB stars in purple, where {\tt fbhb} is increased from 0 to 0.1, 0.5 and 1.0. Allowing hotter BHB stars does not change the ionizing photon budget but does change the UV colors dramatically. 

The addition of blue straggler stars is shown in blue, where we have increased the specific frequency {\tt sbss} from 0 to 0.1, 1, and 5. These stars are not as hot as the BHB stars, and primarily change the NUV flux. In older populations, as the main sequence turn-off evolves to cooler temperatures, the NUV contribution from BS stars should decrease.

%GCs with mostly blue HBs (asterisks) have stronger Balmer lines and thus appear younger than GCs with red HBs (open circles), even though they are all equally old Schiavon
%old hot stars that may be sufficiently bright and numerous to boost the EWs of Balmer lines, mimicking the signature of young stars in the integrated spectra of old SPs.

%-------------------------------------------------------
% Diff stellar types
%-------------------------------------------------------
\begin{figure*}
  \begin{center}
    \includegraphics[width=0.7\textwidth]{figs/f13.png}
    \caption{The UV spectrum of a solar-metallicity instantaneous burst where the contribution of post-AGB stars (orange), blue HB stars (purple), and blue straggler stars (blue) are varied. The unmodified spectrum is shown in black. The post-AGB stars are responsible for the ionizing radiation responsible for producing LIER-like emission, but have little influence over the galaxy's UV colors. In contrast, the blue HB stars and blue straggler stars significantly change the UV color of the population but have little effect on the ionizing radiation output.}
    \label{fig:HPHB}
  \end{center}
\end{figure*}
%-------------------------------------------------------

\subsection{UV-upturn colors}

Fig.~\ref{fig:HPHB} suggests that the FUV and NUV properties of early type galaxies will be sensitive to the details of the post-AGB, HB, and BS populations. Models of ETG UV emission will therefore depend on exactly how these models are implemented. We first compare our baseline ETG models to GALEX observations. We then consider variations in the default \FSPS parameters that bring the models and observations into better alignment.

In Fig.~\ref{fig:UVcolors} we show the $FUV-NUV$ \emph{\vs} $NUV-r$ color evolution of our baseline ETG models as a function of SFH, age and metallicity. Just as in Fig.~\ref{fig:optCols}, each row shows a different SFH, from $\tau=0$, an instantaneous burst, to $\tau$=1\Gyr. The points are color-coded by their metallicity, and the model age is indicated by the opacity, where 13\Gyr models points are fully opaque. The left column shows models that do not include nebular emission, while the right column shows models that include the contribution from nebular line and continuum emission, assuming an ionization parameter of \logUeq{-4}.

Fig.~\ref{fig:UVcolors} is a reproduction of a figure presented in \citet{Hernandez+2014}. To appropriately compare with the \citet{Hernandez+2014} results, we adopt the same observational cut of \hb$\leq 2.1$\ang used in their work on our models. The vertical dashed line at $NUV-r$=5.4 is their galaxy red sequence limit and the horizontal line at $FUV-NUV$ = 0.9 shows the limit for selection of classical UV- upturn galaxies. Galaxies on the red sequence that fall below this line are said to have a ``UV excess'' (UVX) \citep{Smith+2014}. Galaxies below this line but on the blue side of the red sequence division are thought to have blue colors originating from residual star-formation (RSF), rather than canonical UVX emission.

The grey region in Fig.~\ref{fig:UVcolors} shows the range of UV colors observed for ETGs in the \citet{Hernandez+2014} sample. This region is most easily populated by models with high metallicity or somewhat extended SF. Though our models had very similar optical colors, they show a wide range of UV colors in Fig.~\ref{fig:UVcolors}, primarily driven any amount of recent star formation. The sustained star formation in the delayed-$\tau$ models with $\tau$=1\Gyr limited the range of ages and metallicities that could produce ETG-like colors. In Fig.~\ref{fig:UVcolors}, most of these models fall in the ``residual star formation'' section of the diagram.

We note that most of our default models (\emph{left column}) are slightly too red in $FUV-NUV$ to adequately match the \citet{Hernandez+2014} sample. This is slightly improved if we consider the models that include nebular emission (\emph{right column}), which are able to reproduce a wider range of observed ETG colors. At low metallicity however, the models with nebular emission are too blue in $NUV-r$, masquerading as galaxies with residual star formation despite their low \hb equivalent widths and old ages.

\citet{Hernandez+2014} found it difficult to generate models in the UVX portion of the UV color-color diagram without invoking binary star interactions, which can strip the outer envelope of a star, making it appear hotter. In contrast, our models are able to populate the UVX portion of Fig.~\ref{fig:UVcolors}, but only at high metallicity. It is easier to populate the UVX portion of the color-color diagram when including nebular emission, though none of our models reach the most extreme regions of the UVX region.

The default models in Fig.~\ref{fig:UVcolors} do not include BHB or BS populations, (i.e., {\tt fbhb}, {\tt sbss} $= 0$). Including these populations will add flux to the FUV and NUV bands, making $NUV-r$ and $FUV-NUV$ colors bluer. It thus seems likely that post-AGB stars are not solely responsible for the observed UV-excess in ETGs. This points to a scenario where the post-AGB stars produce the ionizing radiation necessary for LIER-like emission, while a different population of HPHB stars drive the FUV and NUV behavior.

%-------------------------------------------------------
% UV colors
%-------------------------------------------------------
\begin{figure*}
  \begin{center}
    \includegraphics[width=0.65\textwidth]{figs/f14.png}
    \caption{$FUV-NUV$ \vs NUV - r colors for our ETG models with stellar only (\emph{left column}) and stellar+nebular emission (\emph{right column}). Each row shows a different delayed$-\tau$ model: $\tau=0.0$\Gyr (instantaneous burst, \emph{top row}), $\tau=0.1$\Gyr (\emph{second row}), $\tau=0.5$\Gyr (\emph{third row}), and $\tau=1$\Gyr (\emph{bottom row}). Models with ages between 1 and 13\Gyr are plotted, color-coded by metallicity. Age is indicated by the transparency of the points, with the 13\Gyr model points fully opaque.
    The vertical dashed line at $NUV-r$=5.4 separates red-sequence galaxies, and the horizontal line at $FUV-NUV$=0.9 shows the boundary of classic UV-upturn galaxies from \citet{Smith+2014}. \citet{Hernandez+2014} further separates strong UV emitters with a FUV-r cut, shown with the grey line. To compare our models with the sample of ETGs from \citet{Hernandez+2014}, we have made the same cut in \hb equivalent width (\hb$<2.0$\ang) in our models. The inclusion of nebular line and continuum emission shifts models to both bluer $FUV-NUV$ and $NUV-r$ colors. The post-AGB stars responsible for nebular emission cannot be wholly responsible for the UV excess in some ETGs.
    }
    \label{fig:UVcolors}
  \end{center}
\end{figure*}
%-------------------------------------------------------

We show the same UV color-color diagram from Fig.~\ref{fig:UVcolors} in Fig.~\ref{fig:UVhphb}V, except now for models where we vary the various HPHB populations. We show instantaneous bursts at 8 and 13\Gyr (left and right panels, respectively), and metallicities of \logZeq{-0.5}, 0.0, and 0.25. The baseline model from Fig.~\ref{fig:UVcolors} is shown in black, for comparison. Variations due to changes in {\tt pagb} are shown in orange, changes in {\tt fbhb} are shown in purple, and changes in {\tt sbss} are shown in blue.

Variations in {\tt sbss} produce negligible changes in the ionizing spectrum at 8 and 13\Gyr, because at these late ages, the rejuvenated main sequence stars are too cool to contribute significantly to the UV flux. Variations in {\tt pagb} parameter move the models away from the observed locus of ETGs, while variations in {\tt fbhb} move the models towards the center of the observed ETG locus. For some models, even a small fraction of BHB stars (${\sim}10$\%) can successfully move the model into the UVX portion of the diagram. However, for most models, increasing {\tt fbhb} largely moves the models to bluer $NUV-r$ colors at similar $FUV-NUV$ colors, indicating that the BHB stars considered here are not hot enough to explain all ETGs with UVX emission. We note that in \FSPS, the BHB stars are evenly distributed across the horizontal branch in temperature. Models with only BHB or EHB stars could still produce the necessary FUV flux needed to move the baseline models into the UVX region.

%-------------------------------------------------------
% UV colors
%-------------------------------------------------------
\begin{figure*}
  \begin{center}
    \includegraphics[width=0.95\textwidth]{figs/f15.png}
    \caption{$FUV-NUV$ \vs NUV - r colors for our ETG models for an instantaneous burst at 8\Gyr (\emph{left}) and 13\Gyr (\emph{right}). Models are connected by lines that are color-coded by metallicity, for \logZeq{-0.5}, 0.0, and 0.25. The black marker indicates the standard stellar population, where {\tt pagb}$\,=1$ and {\tt fbhb}$\,=0$. The varying blue markers show the change in color when {\tt fbhb} is varied from the fiducial model, and the orange colored points show the change in color when {\tt pagb} is varied from the fiducial model.
    The vertical dashed line at $NUV-r$=5.4 separates red-sequence galaxies, and the horizontal line at $FUV-NUV$=0.9 shows the boundary of classic UV-upturn galaxies from \citet{Smith+2014}. \citet{Hernandez+2014} further separates strong UV emitters with a FUV-r cut, shown with the grey line.
    }
    \label{fig:UVhphb}
  \end{center}
\end{figure*}
%-------------------------------------------------------

\section{Isochrone variations}

In \S\ref{sec:stars} we demonstrated that the MIST models are able to simultaneously reproduce the optical colors and nebular emission properties of LIER-like galaxies for a range of ages, SFGs, and metallicities. Post-AGB stars are the sole provider of ionizing photons in these models. In the MIST models, the evolution of stars at all masses is continuously computed, from the pre-main sequence phase to the end of white dwarf (WD) cooling phase. This means that we can directly probe the sensitivity of post-AGB star evolution to the various default assumptions in the evolutionary tracks.

In this section we explore modifications to the MIST models that affect the duration and intensity of the post-AGB phase to test how this alters the resultant nebular emission. We test three variants: overshoot mixing efficiency, mass loss, and rotation rate. We briefly describe each of these variants in turn.

\paragraph{Overshoot mixing efficiency} In the MIST models, the convective mixing of elements in the stellar interior is implemented using the mixing length theory (MLT) formalism, described at length in \citet{Choi+2016}. The mixing is a time-dependent diffusive process, which is modified by overshoot mixing across convection boundaries. The overshoot action leads to enhanced mixing, and is used to account for the observed properties of AGB and post-AGB stars \citep{Herwig+2000}. The method adopted by MIST follows the parametrization of \citet{Herwig+2000}, which modifies the diffusion coefficient in the overshoot region through an exponentially decaying diffusion process. The efficiency of that decay is set by $f_{ov}$, a free parameter that determines the efficiency of overshoot mixing. In this work we use MIST variants where the efficiency of overshoot mixing in the envelope of thermally pulsing (TP)-AGB stars has changed. The default MIST model has $f_{\mathrm{ov, env}}=$0.0174. Our modified model has $f_{ov}=$0.0052, corresponding to a 30\% decrease in mixing efficiency. We refer to this model as {\tt MIST\_DUPx0.3}.

\paragraph{Rotation} The MIST models include the effect of rotation, discussed at length in \citet{Choi+2017}. The effects of rotation appear in the MESA stellar evolution calculations in three main ways. First, rotation decreases the gravitational acceleration via the centrifugal force, which in turn affects the stellar structure. Second, rotation can promote extra mixing in the interior, boosting the transport of chemicals and angular momentum. MESA adopts the common approach of treating the chemical and angular momentum transport in a diffusion approximation. Third, rotation enhances mass loss. MESA adopts the formulation from \citet{Langer+1998}, where the mass loss rate $\dot{M}$ is multiplied by a factor that increases dramatically as the surface angular velocity $\Omega$ approaches critical, or break-up, angular velocity. The default MIST model assumes an initial rotation rate of  $\nu_{\mathrm{ZAMS}}/\nu_{\mathrm{crit}} = 0.4$, meaning that the the surface velocity is set to 40\% of the critical, or break-up, velocity. In this work we use MIST variants where the rotation rate is increased to $\nu_{\mathrm{ZAMS}}/\nu_{\mathrm{crit}} = 0.6,0.8$ ({\tt MIST\_vvcrit0.6} and {\tt MIST\_vvcrit0.8}, respectively).

\paragraph{Mass Loss} We use MIST variants related to mass loss. In the first, both $\eta_M$ and $\eta_B$, the mass loss efficiency factors for the RGB and AGB, respectively, are decreased by half ({\tt MIST\_mdotx0.5}). In the second, both $\eta_M$ and $\eta_B$ are doubled ({\tt MIST\_mdotx2}).

\paragraph{} We run each of the above MIST variants through \Cloudy at solar metallicity using identical input parameters. In Fig.~\ref{fig:EWvar}, we show the resultant \ha equivalent widths produced by the MIST variants at 8\Gyr for a range of ionization parameters. The format of Fig.~\ref{fig:EWvar} is similar to that in Fig.~\ref{fig:EWtau}, where each pixel represents a different model. The $x$-axis shows each of the MIST variants, where the fiducial column represents the standard MIST model. The $y$-axis shows ionization paramter, which varies from \logUeq{-6} to -3. The \ha equivalent widths vary from 0.42 to 0.66\ang. Unsurprisingly, all the MIST variants show \ha equivalent widths that increase as \logU is increased. 

The MIST variants show a range of behaviors when compared to the fiducial model. The model where the overshoot mixing efficiency has been decreased by 30\% (DUP$\times$0.3) shows smaller \ha equivalent widths than the fiducial model, though only by a few percent.

The models where the mass loss efficiency factors show different emission properties. The model with less efficient mass loss has smaller equivalent widths than the fiducial model at all ionization parameters. In contrast, the model with increased mass loss efficiency shows enhanced equivalent widths when compared to the fiducial model. 

The models with increased rotation rates show very little change compared to the fiducial model. This is not unexpected, since rotation plays an important role for young, massive stars but has minimal effect on the TP-AGB to post-AGB transition.

%-------------------------------------------------------
% Tau models: Ha EW time evolution
%-------------------------------------------------------
\begin{figure*}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figs/ftemp3.pdf}
    \caption{For solar metallicity models at 8\Gyr and \logUeq{-4}, we show the \ha equivalent width for the MIST variations.}
    \label{fig:EWvar}
  \end{center}
\end{figure*}
%-------------------------------------------------------
Enhanced mass loss seems like a promising way enhance the ionizing properties of post-AGB stars. We note that doubling the mass loss efficiency factors is not an unreasonable, the default MIST model uses $\eta_{\mathrm{R}} = 0.1$ and $\eta_{\mathrm{B}} = 0.2$, which increases to $\eta_{\mathrm{R}} = 0.2$ and $\eta_{\mathrm{B}} = 0.4$, respectively, in the {\tt MIST\_mdotx2} model. Mass loss efficiency parameters as high as 0.8 have been suggested in some cases. %(XXXcite).


\item For the standard set of models presented here, we find that the UVX region of the $FUV-NUV$ versus $NUV-r$ diagram can only be populated by high metallicity models. Populating the UVX region is easier with models that include nebular emission. Models with high metallicity and somewhat extended SF are most easily able to reproduce the observed UV colors from \citet{Hernandez+2014}.

\item Post-AGB stars can drive LIER-like emission and contribute to the UV-excess observed in ETGs. It is more likely, however, that the UVX is driven by a small population of alternative HPHB stars, like blue horizontal branch stars. These stars do not contribute significantly to the ionizing photon budget of evolved stellar populations, but can change the UV colors by orders of magnitude.

\item We have tested the sensitivity of the post-AGB phase to several of the default parameters used in the MIST models. We have found that rotation has a negligible affect on the ionizing properties of post-AGB stars. We have found that increasing the mass loss efficiency increased the resultant \ha equivalent widths and decreasing the mass loss efficiency decreased the resultant \ha equivalent widths from the fiducial model. This is a promising area to explore in future work. 




%-------------------------------------------------------
% Tau models: LINEAR Ha EW time evolution
%-------------------------------------------------------
\begin{figure*}
  \begin{center}
    \includegraphics[width=\linewidth]{figs/f13.png}
    \caption{\emph{Top:} The time evolution of \ha equivalent widths for the subset of models with optical colors consistent with the general ETG population. The columns show $\tau=0.1$\Gyr (\emph{left}),  $\tau=0.5$\Gyr (\emph{middle}), and $\tau=1.0$\Gyr (\emph{right}). Metallicity varies from \logZeq{-2} in dark purple to \logZeq{0.5} in yellow; only the models with metallicities above \logZeq{-1.0} have ETG-like colors and LIER-like EWs. \emph{Bottom:} \ha equivalent widths as a function of metallicity for for $\tau=0.1$\Gyr (\emph{left}),  $\tau=0.5$\Gyr (\emph{middle}), and $\tau=1.0$\Gyr (\emph{right}). Ionization parameter is varied from \logUeq{-6} in light blue to \logUeq{-3} in dark blue. The subset of models with consistent ETG colors are highlighted with the circle markers.}
    \label{fig:linearEW}
  \end{center}
\end{figure*}
%-------------------------------------------------------


%We compare the \ha equivalent widths as a function of time for the delayed-$\tau$ models in Fig.~\ref{fig:EWtau}. Each panel shows a different model SFH at a range of metallicities, assuming \logUeq{-4}. For the models at \logUeq{-4}, the equivalent widths range from 0.1 to 5\ang at ages 1\Gyr and older. Larger values of $\tau$ produce a larger range in \ha EWs, especially at younger ages.

%As shown in Figs.~\ref{fig:optCols}-\ref{fig:LickHb}, the main effect of SFH is to change the age at which a model looks like an ETG. Larger values of $\tau$ extend the duration of SF in a model, and these models do not look like ETGs until much later than the instantaneous bursts. The instantaneous bursts have ``ETG-like'' colors after $\sim3$\Gyr, while the models with $\tau$=1\Gyr only have ``ETG-like'' colors after 8\Gyr. The large EWs found in the $\tau$=1\Gyr models of Fig.~\ref{fig:EWtau} (right panel) are associated with contamination from residual star formation.

%We have demonstrated that there are a broad range of model ages, SFHs, and metallicities that are able to reproduce the optical colors and absorption indices of ETGs. We now assess the emission line properties of the subset of models with optical spectra that ``look'' like ETGs. For the full grid of models that include nebular emission, we determine if the resultant broad-band colors are consistent with the observed range of ETGs, as determined using the region shown in Fig.~\ref{fig:optCols}, defined by \citet{Holden+2012} and updated by \citet{McIntosh+2014}.

%We show \ha EWs for the delayed-$\tau$ models with ``ETG-like'' optical properties in Fig.~\ref{fig:linearEW}. The top panel shows the time evolution of \ha equivalent widths at several metallicities, masking out all models that do not have ETG-like colors. Only models with metallicities of \logZeq{-1} and higher have colors consistent with the general ETG population. These models have \ha equivalent widths that vary from 0.1 to 3\ang with age, metallicity, and SFH.

%The lower left panel of Fig.~\ref{fig:linearEW} shows the variation of \ha equivalent widths with metallicity, for models at $\log t = 10$ (10\Gyr) and a range of ionization parameters. We highlight those models with ETG-like colors with circular markers. For $\tau$=0.1 and 0.5\Gyr, the range of \ha equivalent widths is quite small, varying from 0.5 to 1\ang. For stellar populations at all metallicities, the post-AGB population has very similar temperatures, producing ionizing spectra with similar hardness. We thus expect that the models have similar ionization states, producing similar emission line ratios, as demonstrated in Fig.~\ref{fig:BPT}. 

%Metallicity does change the emission properties of the models in two subtle ways. First, metallicity changes the underlying stellar continuum, and thus the \ha equivalent width. As shown in Fig.~\ref{fig:ionSpec}, lower metallicity models are brighter and hotter in the optical, and will have a larger contribution from the continuum. For a fixed number of ionizing photons, a larger continuum contribution produces smaller equivalent widths. Fig.~\ref{fig:EWtau} shows some evidence of larger EWs in higher metallicity models. Second, the lower metallicity models have more ionizing photons per unit stellar mass, and will thus produce more \ha emission. Fig.~\ref{fig:EWtau} shows some evidence of larger EWs at the lowest metallicities, but we note that these models do not produce optical colors that are consistent with the general ETG population.

%Fig.~\ref{fig:linearEW} also shows the variation of the \ha equivalent width as a function of ionization parameter. The behavior is as expected here, where models with higher ionization parameters produce larger \ha equivalent widths. However, the range of EW is quite modest in spite of the large variation in \U, with the \ha EWs varying by only 15\% as the ionization parameter changes by 2 orders of magnitude. This suggests that although \U is a significant uncertainty in our physical model, the predictions of \ha EWs are relatively insensitive to the exact value of \U. In the model with $\tau$=1\Gyr, variation in ionization paramter produces a larger range in \ha EWs, due to the residual star formation.


%-------------------------------------------------------
% Tau models: Ha EW time evolution
%-------------------------------------------------------
%\begin{figure*}
%  \begin{center}
%    \includegraphics[width=\linewidth]{figs/f12.png}
%    \caption{The time evolution of \ha equivalent widths for the delayed-$\tau$ models for $\tau=0.1$\Gyr (\emph{left}),  $\tau=0.5$\Gyr (\emph{middle}), and $\tau=1.0$\Gyr (\emph{right}). Metallicity varies from \logZeq{-2} in dark purple to \logZeq{0.5} in yellow. The grey shaded region highlights \ha EWs observed in typical LIER-like galaxies, of order $0.1-3\,$\ang.}
%    \label{fig:EWtau}
%  \end{center}
%\end{figure*}
%-------------------------------------------------------

%To briefly summarize, our models that include nebular emission are able to reproduce the optical properties of the general ETG population over a range of ages, SFHs, and metallicities. We find that instantaneous bursts and delayed-$\tau$ models with $\tau$=0.1, 0.5\Gyr, ages older than 3\Gyr, and metallicities between \logZeq{-1} and \logZeq{0.25} produce the most consistent combination of optical colors and Lick indices when compared with ETGs. This same subset of models produces \ha equivalent widths of order 0.1-3\ang, consistent with LIER-like galaxies. We find some evidence for higher \ha equivalent widths in higher metallicity models and models with higher ionization parameters, but in general the \ha EW is far more sensitive to age and SFH than either metallicity or \U.


%To best reproduce observed LIER-like emission line ratios, models with older ages (5-10\Gyr), low gas densities ($n_{\mathrm{H}}\sim 1-10$ cm$^{-3}$), and moderate ionization parameters ($-5<\logU<-3$) are preferred.
%While stellar metallicity has little effect on the emission line ratios, it does change the equivalent widths, as seen in Figs.~\ref{fig:EW} \& \ref{fig:EWtau}, but largely through the properties of the continuum, rather than the emission lines.

%In summary, Figures~\ref{fig:EW} - \ref{fig:BPT} indicate that our models produce emission line ratios that agree well with those observed in LIER-like galaxies, with no fine tuning needed to produce acceptable models. % Their optical colors and line indices are consistent with ETGs and simultaneously produce emission line equivalent widths and emission line ratios observed in LIER-like galaxies. 

% Lower overshoot efficiency results in shorter MS lifetimes and systematically lower MSTO masses and luminosities. SGB and CHeB luminosities are lower due to the resulting smaller core masses. Core overshoot efficiency is constrained by matching the MSTO in M67, and the envelope overshoot efficiency is determined during solar calibration.

% The morphology of the CHeB is directly influenced by mass-loss rates: lower and higher mass-loss rates yield hotter and cooler CHeB, respectively. Mass-loss rates should also affect the TP AGB phase, because more efficient winds will lead to fainter and fewer TPs.

